Accelerating LSTM-based High-Rate Dynamic System Models

In this paper, we evaluate the use of a trained Long Short-Term Memory (LSTM) network as a surrogate for a Euler-Bernoulli beam model, and then we describe and characterize an FPGA-based deployment of the model for use in real-time structural health monitoring applications. The focus of our efforts is the DROPBEAR (Dynamic Reproduction of Projectiles in Ballistic Environments for Advanced Research) dataset, which was generated as a benchmark for the study of real-time structural modeling applications. The purpose of DROPBEAR is to evaluate models that take vibration data as input and give the initial conditions of the cantilever beam on which the measurements were taken as output. DROPBEAR is meant to serve an exemplar for emerging high-rate "active structures" that can be actively controlled with feedback latencies of less than one microsecond. Although the Euler-Bernoulli beam model is a well-known solution to this modeling problem, its computational cost is prohibitive for the time scales of interest. It has been previously shown that a properly structured LSTM network can achieve comparable accuracy with less workload, but achieving sub-microsecond model latency remains a challenge. Our approach is to deploy the LSTM optimized specifically for latency on FPGA. We designed the model using both high-level synthesis (HLS) and hardware description language (HDL). The lowest latency of 1.42 $\mu$S and the highest throughput of 7.87 Gops/s were achieved on Alveo U55C platform for HDL design.

==> background.tex <==
\section{Background on LSTM}\label{back}

% JDB: do we need to cite the source of Fig. 1? E.K: No, it is my drawing.

The operations within a basic LSTM cell is shown in Fig.~\ref{LSTM}. It shows how matrix vector multiplication, element-wise multiplication and addition and activation functions are applied on the input vectors ($x_{t}$), hidden state vectors ($h_{t}$), input weight matrices ($W_{x}$), recurrent weight matrices ($W_{h}$), bias vectors ($b$) and cell state vectors ($c_{t}$). %The input and hidden state vectors are concatenated so that the weight matrix holds both input weights and recurrent weights.
\begin{figure}[h!]
\centering
%\includegraphics[width=1\linewidth]{figures/arch-n.png}
\includegraphics[height=4cm, width=0.9\linewidth]{figures/lstm2.png}
\caption{\label{LSTM}General LSTM Cell}
\end{figure}
%\vspace{-0.4cm}
\begin{equation}
    i_t = \sigma(W_{ix}X_t + W_{ih}h_{t-1} + b_i)
\end{equation}
\begin{equation}
    f_t = \sigma(W_{fx}X_t + W_{fh}h_{t-1} + b_f)
\end{equation}
\begin{equation}
    u_t = \tanh(W_{cx}X_t + W_{ch}h_{t-1} + b_c)
\end{equation}
\begin{equation}
    o_t = \sigma(W_{ox}X_t + W_{oh}h_{t-1} + b_o)
\end{equation}
\begin{equation}
    c_t = f_t\odot{c_{t-1}} + i_t\odot{u_{t}}
\end{equation}
\begin{equation}
    h_t = o_t\odot{\tanh{(c_t)}}
\end{equation}

All operations in Fig.~\ref{LSTM} can be expressed by Eqs. (1) to (6) above. \textit{i}, \textit{f}, \textit{u} and \textit{o} represent the input gate, the forget gate, the input modulation gate, and the output gate respectively at time step \textit{t}. $h_{t}$ and $c_{t}$ are passed to the next time step of the same layer or to the next layer. The symbols $\sigma$, $\tanh$, and $\odot$ are sigmoid function, the hyperbolic tangent function, and element-wise multiplication respectively.

==> data_representation.tex <==
\begin{comment}
\section{Performance Defining parameters}
\subsection{Data Representation}
%\emph{dla-kind of clunky}
The specific data precision and representation can have a significant effect on performance, area, and accuracy. In our design, we allow floating point or fixed point representations to be specified before synthesis.  Floating point computations are slower and consume more area compared to fixed point computations, but will provide wider range.  Hence the trade-off among the three parameters could decide the data representation. When fixed point is chosen, the word length (bit precision) for the inputs, weights, and outputs need to be considered to avoid overflow. Fixed point data type is represented by (s, ws, fl) where `s' is the sign bit, `ws' is the word length, and `fl' is the fraction length. The range and precision of a fixed point number depend on the word length. The precision is the difference between two neighboring representable values, which is equals to $2^{-fl}$.
In the  CNN-MLPA, the fixed point size must be scaled based on some configuration parameters of the maximum network topology such as Maximum Number of Layers (MNL), Maximum Number of Neurons (MNN), Maximum Number of Neurons in Largest Layer (MNNLL), Maximum Number of Inputs (MNI), and Maximum Number of Outputs (MNO) following equation (1) and (2).
\begin{equation}
 n_c = max(MNI,MNNLL)
 \end{equation}

\begin{equation}
n_{s}=log_{2}(n_c\times(2^{n_{z}-1}-1)\times(2^{n_{w}-1}-1)) +1
 \end{equation}

where $n_c$: maximum  number of incoming connections to a neuron (fan-in),
$n_s$: number of bits of the weighted sum,
$n_z$: number of bits of a neuron inputs and outputs, and
$n_w$: number of bits of weights. Details about fixed point size scaling can be found in \cite{Omondi,Moussa}.
%
%\emph{dla-is this next sentence supposed to be generic or describe your design ?}
%The MLPCP presented in this paper is designed with flexibility in mind, to allow a range of topologies to be created by setting the following parameters: Maximum Number of Layers (MNL), Maximum Number of Neurons (MNN), Maximum Number of Neurons in Largest Layer (MNNLL), Maximum Number of Inputs (MNI), and Maximum Number of Outputs (MNO). 



%Therefore, it is necessary to choose the word length of the inputs, outputs (both with same number of bits), weights based on the following formulas:

%
% two equations


% insert a figure here. (sampling log sigmoid and tan sigmoid)
 
 \subsection{Activation Functions}
Activation Functions (AFs) range from simple step functions to more complex sigmoid functions. Sigmoid functions are the most frequently used in DNNs \cite{Misra}. Clearly, a step function \cite{reluweb} shown in formula~\ref{relu}
is easy to implement within an FPGA as it produces only one of the two values based on a specific threshold.  In contrast, the log-sigmoid %and tan-sigmoid 
function shown in formula~\ref{sigmoid}\cite{sigmoid}
% and \ref{tansigmoid} \cite{tangent} respectively 
require more resources to implement compared to the simple step function.  Several approaches have been proposed to reduce the resource requirements of implementing 
AFs on FPGAs.  Hikawa \cite{Hikawa} proposed a digital pulse mode neuron that employs a piecewise linear function as its activation function. Daalen et al.\cite{Shawe,Daalen} 
demonstrated through experiments how linear and sigmoid AFs can be generated in a digital stochastic bit stream neuron. However, computation-based AFs consume a lot of resources; hence, the 
common way to implement sigmoid function is to use LUTs, which is faster and requires fewer resources with a reduced accuracy.  Our CNN-MLPA provides two options to realize AFs: 
computation-based AF (using high level synthesis), or LUT-based AF. For example, if the sampling interval is [-1, 1] with step size $\Delta$x = 0.1 for log-sigmoid, %and tan-sigmoid
20 samples will be produced occupying 20 memory locations for each AF. Then the AF's output will be `0' in log-sigmoid for the input values less than `-1' and the output will be `1' for input values more than `1'.
%AF and `-1' in tan-sigmoid AF 
%the output for the input values which were more than `5' were set to `1' for both log-sigmoid and tan-sigmoid. both log-sigmoid and tan-sigmoid  AF 
%Resource utilization and performance results for both are reported in result section (5).

\begin{equation} 
 step(x)=max(0,x)
 %\frac{e^{2x}-1}{e^{2x}+1}=1-\frac{2}{e^{2x}+1} 
 \label{relu}
 \end{equation}

\begin{equation}
 sigmoid(x)=\frac{1}{1+e^{-x}}
 \label{sigmoid}
 \end{equation}
 
 
 
 
 
 %%% \begin{equation}
 %%% Y(x)=\frac{e^{x}-e^{-x}}{e^{x}+e^{-x}}
%%% \end{equation}
\hfill
%
\end{comment}

==> dynamics.tex <==
\section{High-Rate Dynamic Events}\label{dynamics}

High-rate dynamic environments refer to environments in which structures are subjected to impact loading that results in accelerations greater than 100 g for time periods of less than 100 ms \cite{Hong2018IntroductionStateEstimation}. Space infrastructure and blast mitigation systems are examples of structures experiencing high-rate dynamic events. Systems exposed to such environments require rapid response, from event detection to decision-making, in the sub-millisecond scale to ensure safe and reliable operations. Traditional control strategies like finite element model-based state-estimation algorithms are shown to under-perform when the required resolution of the model exceeds the computing capacity of the real-time system. The emerging field of High-Rate Structural Health Monitoring (HR-SHM) and Prognostics is focused on control systems that are made possible by the recent introduction of real-time sensing, edge computing, and high-bandwidth computer memory \cite{high-rate5}.

